Single copy of the Ricci flow

The perturbative double copy is by now a highly established correspondence between gravity and gauge theories. Non-perturbatively, information ranging from classical solutions to topological quantities on both sides have been related to each other via the double copy correspondence. In this paper, we add another result, where we show that the single copy of the Ricci flow is the Yang-Mills flow on the space of connections of a principal $\text{U}(1)$-bundle.

==> sections/__latexindent_temp.tex <==
Given our choice of applying the Kerr-Schild single copy on a flat minkowski background, equation \eqref{YMFlow} should be interpreted as the flow in the space of connections of a $\text{U}(1)$ principle bundle $(P,\mathbb{R}^{1,d-1},\text{U}(1))$ with curvature $F = d(X,Y)\circ \text{hor}$ for vectors $X,Y\in TE$. Again, eq. \eqref{YMFlow} is analogous to a diffusion equation for the gauge field $A_{\mu}$ since if we use $F_{\mu\nu} = 2\pd_{[\mu}A_{\nu]}$ we have
